HumanGAN: A Generative Model of Humans Images

Generative adversarial networks achieve great performance in photorealistic image synthesis in various domains, including human images. However, they usually employ latent vectors that encode the sampled outputs globally. This does not allow convenient control of semantically-relevant individual parts of the image, and is not able to draw samples that only differ in partial aspects, such as clothing style. We address these limitations and present a generative model for images of dressed humans offering control over pose, local body part appearance and garment style. This is the first method to solve various aspects of human image generation such as global appearance sampling, pose transfer, parts and garment transfer, and parts sampling jointly in a unified framework. As our model encodes part-based latent appearance vectors in a normalized pose-independent space and warps them to different poses, it preserves body and clothing appearance under varying posture. Experiments show that our flexible and general generative method outperforms task-specific baselines for pose-conditioned image generation, pose transfer and part sampling in terms of realism and output resolution.

==> HumanGan_ A Generative Model of Humans - arxiv/Sections/abstract.tex <==
Generative adversarial networks achieve great performance in photorealistic image synthesis in various domains, including human images. 
%
However, they usually employ latent vectors that encode the sampled outputs globally.
% 
This does not allow convenient control 
of semantically-relevant individual parts of the image, and cannot draw  samples that only differ in partial aspects, such as clothing style. 
% 
%
We address these limitations and present a generative model for images of dressed humans offering control over pose, local body part appearance and garment style. 
%To the best of our knowledge, 
This is the first method to solve various aspects of human image generation, such as global appearance sampling, pose transfer, parts and garment transfer, and part sampling jointly in a unified framework. 
% 
As our model encodes part-based latent appearance vectors in a normalized pose-independent space and warps them to different poses,  it preserves body and clothing appearance under varying posture. 
% 
Experiments show that our flexible  and  general  generative method outperforms task-specific baselines for pose-conditioned image generation, pose transfer and part sampling in terms of realism and output resolution.
% 

==> HumanGan_ A Generative Model of Humans - arxiv/Sections/discussion.tex <==
 
\section{Limitations and Future Work}
%\noindent\textbf{Limitations and Future Work.} 
% We have found that 
Our method sometimes demonstrates spurious interleaving of body parts or garments in the generated images (\textit{e.g.,} see  Fig.~\ref{fig:latent_inter}, right-most images). 
% 
However, this is also shared by other (less realistic) generative human models (see the result of VUNet in  Fig.~\ref{fig:appearance} and the baselines in Fig.~\ref{fig:transfer}). These artifacts could be avoided by a hierarchical generator, where the garment style is generated first. This design, however, comes with the disadvantage of not being able to perform part-based sampling. We have also found that our generated images are biased towards females. This, we hypothesize, is due to the bias in the DeepFashion dataset. 



\textit{garment transfer} between two images representing the body and garments. To this end, we first encode the appearance of both the body image $\bm I_b$ and garment image $\bm I_g$, in their part-based noise vectors $\bm z_b$ and $\bm z_g$ receptively. We then construct a new noise embedding that comprises of the body parts $\bm z_b[p] \mid p \in$ \textit{Body}, and garment parts $\bm z_g[p] \mid p \in$ \textit{Garments} of the two noise embeddings, and use it in the generator for the final output, see
% . Our results are shown in 
Fig.~\ref{fig:garments}. 

\section{Conclusion} 
\label{sec:conclusion} 
% 
We  have presented a generative model for full-body images of clothed humans, which enables control of body pose, as well as independent control and sampling of appearance and clothing style on a body part level. 
% 
A framework based on variational autoencoders is used to induce stochasticity in the appearance space. 
% 
To achieve the disentanglement of pose and appearance, we encode the posterior probability of the part-specific latent vectors from a space of pose-independent appearance and warp the encoded vector to a different pose before performing the reconstruction. 
% 
Experiments with pose-conditioned image generation, pose transfer, as well as parts and garment transfer, have demonstrated that the model improves over the state-of-the-arts. 
% 

\noindent\textbf{Acknowledgements.} This work was supported by the ERC Consolidator Grant 4DReply (770784) and Lise Meitner Postdoctoral Fellowship. 
% 
We thank Dushyant Mehta for the feedback on the draft. 
% 


==> HumanGan_ A Generative Model of Humans - arxiv/Sections/introduction.tex <==
%!TEX root = ../article.tex
\section{Introduction}
\label{sec:intro}

%\blfootnote{Project webpage:  \url{gvv.mpi-inf.mpg.de/projects/HumanGAN/}}

Algorithms to generate images of clothed humans find many applications in such fields as virtual and augmented reality, data generation and augmentation for neural network training. 
% 
%\VG{add a couple of references supporting the claim} 
% 
For content creation, it is often desired to have full control over semantic properties of the generated images (\textit{e.g.,} pose, body appearance and garment style). 
% 
One way of achieving this is to use computer graphics with precise control over the image rendering. 
%
However, creating just a single photo-realistic image in this way is challenging and tedious and requires expert knowledge in 3D modeling,  animation and rendering algorithms. 


Recently, generative adversarial networks (GANs) have made significant progress in generating photo-realistic images, which can also be applied to synthesize imagery of humans 
\cite{Brock2018Biggan,karras2018progressive,karras2019style,Karras2019stylegan2}.  
% 
These methods learn a mapping from an easy-to-sample latent space that can be sampled to the image domain and is able to synthesize photo-realistic imagery  without the need to resort to complex compute graphics style modeling and light transport simulation. 
%making them an excellent choice as a generative model. 
% However, 
A limitation of these generative models from a content creation perspective is that, in contrast to computer graphics synthesis, they do not easily permit control over  semantic attributes of the output imagery. 
%the generation process doesn't provide control of the output over semantically well defined attributes. 
Recently, Tewari \textit{et al.}~\cite{tewari2020stylerig,tewari2020pie} study StyleGAN \cite{karras2019style} to achieve a rig-like control over 3D interpretable face parameters, such as face pose, expression and illumination. 
% 
However, these methods only work well for faces with limited 3D poses \cite{tewari2020stylerig}, and extending such a method to humans---that relies on differentiable rendering of a 3D morphable model---is not straightforward. 

In a setting related to ours, there has been  significant progress in conditional image generation with explicit inputs of specific control variables \cite{pix2pix2017, wang2018pix2pixHD}. 
%However, these methods of translation networks produce a single output given the conditional input. 
Conditional models of this type that use conditioning inputs from a parametric human body model have shown impressive results in applications such as pose and garment transfer \cite{Sarkar2020,Grigorev2019CoordinateBasedTI,Siarohin2019AppearanceAP,Neverova2018}. 
Unfortunately, their underlying translation network does not constitute a full generative model that can be sampled from, as they are designed to produce a single output deterministically. 



In this work, we present \textit{HumanGAN}, \textit{i.e.,} a novel generative model for full-body images of clothed humans, which enables control of  body pose, as well as independent control and sampling of  appearance and clothing style on a body part level \footnote{project webpage: \url{gvv.mpi-inf.mpg.de/projects/HumanGAN/}}. 
% 
Our method combines the advantages of both worlds,  \textit{i.e.,} the latent-space-based GANs and controllable  translation networks, in the framework of conditional  variational autoencoder \cite{Kingma2014VAE}. 
% 
We encode the true posterior probability of the latent variable from a space of pose-independent appearance and reconstruct a photo-realistic image of the human with a high-fidelity generator using the encoded latent vector. 
% 
To disentangle a pose from local part appearance, we propose a novel strategy where we condition the latent vectors on body parts and warp them to a different pose before performing the reconstruction. 
This permits pose control under persistent appearance and clothing style, and appearance sampling on a localized body part level, without affecting the pose, see Fig.~\ref{fig:teaser}.
To summarize, our \textbf{contributions} are as follows: 
\vspace{-0.2cm}
\begin{itemize}[leftmargin=*]
\itemsep-0.2em
\item HumanGAN, \textit{i.e.,} a new state-of-the-art generalized model for human image generation that can perform global appearance sampling, pose transfer, parts and garment transfer, as well as part sampling. 
For the first time, a \textit{single method} can support \textit{all these tasks} (Sec.~\ref{sec:method}). 
% in the literature 
% 
\item A novel strategy of part-based encoding and part-specific spatial warping in a variational framework that disentangles pose and appearance over the body parts. 
\end{itemize}
% 
\vspace{-0.2cm}
In our experiments (Sec.~\ref{sec:results}), we significantly outperform the state of the art (and other tested methods) for human appearance sampling in realism, diversity and output resolution ($512 \times 512$).
% 
Furthermore, our general model shows commendable results for \textit{pose transfer} that are on par with the state-of-the-art methods developed for this task. 
%Please visit the project webpage:  \url{gvv.mpi-inf.mpg.de/projects/HumanGAN/} for the accompanying video and our results on the DeepFashion dataset.


==> HumanGan_ A Generative Model of Humans - arxiv/Sections/method.tex <==
%!TEX root = ../article.tex
\section{Method}
\label{sec:method}

\begin{figure*}[t] 
    \includegraphics[width=\linewidth]{Figures/pipeline2.png} 
    \caption{Overview of our method. Given a source image $I_s$, we extract human appearance in the form of a UV texture map $T_s$. Subsequently, the Encoder encodes $T_s$ to part specific latent vectors $\bm z_s$. We use the target pose $P_t$ to warp and broadcast the latent vectors to the corresponding part locations in the target image to create a noise image $Z_t$. Finally, the generator converts the noise image to a realistic image. During testing, we generate random samples by controlling the latent vectors $\bf z \in \mathcal{N}(0,1)$ and the target pose $P_t$.}
    %\caption{Overview of our method. Given a source image $I_s$ and target image pair ($I_s, I_t$), we encode the source appearance from a normalized pose independent appearance space $T_s$ to part specific latent vectors $\bf z_s$. We use the target pose $P_t$ to warp and broadcast the latent vectors to the corresponding part locations in the target image and form a noise image $Z_t$. Subsequently, the generator converts the noise image to a realistic image. During testing, we generate random samples by controlling the latent vectors $\bf z \in \mathcal{N}(0,1)$ and the target pose $P_t$.} 
    \label{fig:pipeline} 
\end{figure*} 



%\begin{figure}[t] 
%    \includegraphics[width=\linewidth]{Figures/uv_texture.png} 
%    \caption{Extraction of appearance in the SMPL texture space} 
%    \label{fig:uvtexture} 
%\end{figure} 

%\paragraph{Terminology} 
%Source image, Source Pose  $I_{s}, P_{s}$
%
%Partial Texture map of the input - $T_{s}$
%
%Encoder - \textit{Enc}, E
%
%Target pose - $P_t$.
%
%Warping function - \textit{Warp, W}
%
%Sampled Noise - $\bm z$ (note that the dependence on source $s$ is dropped), tiled noise in the texture space - $T_Z$, Warped noise image - $Z_{t}$.
%
%Generator - \textit{Gen}, \textit{G}
%
%Generated image, on noise Z, and pose t - $I_{Z,t}$
%
%Pipeline can be described by the following equations:
%
%\begin{equation*}\label{eq:pareto mle2}
%  \begin{aligned}
%\mu, \sigma = E(T_s)\\
%Z \sim p(\mu, \sigma)\\
%Z_t = W(P_t, T_z)\\
%I_{Z,t} = G(Z_t)\\
% \end{aligned}
%\end{equation*}

\subsection{Method Overview}
Our goal is to learn a generative model for human images, which is conditioned on body pose and a low dimensional latent vector encapsulating the appearance \LJ{a low dimensional latent vector encapsulating the appearance -> a low dimensional latent vector where each dimension encapsulates the appearance of different body parts?}. 
We use DensePose~\cite{Guler2018DensePose} to represent the human pose because of the ease of use in terms of texture warping, and its popularity in the existing literature \cite{Siarohin2019AppearanceAP,Neverova2018,Grigorev2019CoordinateBasedTI,Sarkar2020} \LJ{should we mention why we use Densepose?}.
Our method can be described by \LJ{revised as: Our task can be formulated as?} a deterministic mapping $G':(\bm P, \bm z) \rightarrow \bm I$. Here, $\bm P \in \mathbb{R}^{H \times W \times 3}$ is a 3 channel DensePose image representing the conditioning pose, $\bm z \in \mathbb{R}^{M \times N}$ is the latent vector comprising of  $M$ human-body-parts and $N$ part-specific latent vector dimensions, and $\bm I \in \mathbb{R}^{H \times W \times 3}$ is the generated output image. 


For learning such function with a latent variable capturing the ambiguous aspect of the output, we build our method on Variational Auto-Encoder (VAE) \cite{Kingma2014VAE}. As in any latent vector model, the observed variable $\bm x$ is assumed to be dependent on an unobserved hidden latent variable $\bm z$ which encode semantically meaningful information about $\bm x$. 
%We adopt the belief that the latent variable $z$ only encode the part specific appearance. 
%The marginal distribution of the observed variable is then given by $p(I) = \int p(I, z) \,dz$. 
The goal of the generative model then is to find the distribution that maximize the marginal log-likelihood $\sum_{\bm x \in p_{\text{data}}} \log \int p_\theta(\bm x|\bm z) p(\bm z) d \bm{z}$ w.r.t. the parameters $\theta$. To make this problem tractable, a distribution $q_\phi(\bm{z|x})$ with learnable parameters, the encoder, is introduced that approximate the true but intractable posterior $p(\bm{z|x})$. With the above formulation and the Gaussian assumption on the distribution $p(\bm z)$ and $q_\phi(\bm{z|x})$, the VAE objective is to minimize $\mathcal{L}_{rec} + \mathcal{L}_{prior}$, where $\mathcal{L}_{rec}$ is the reconstruction loss, and  $\mathcal{L}_{prior}$ the KL divergence on the encoded distribution and the standard normal distribution \cite{Kingma2014VAE}. 

In this work, we use the conditional version of the VAE to learn the joint distribution $p_{\theta}(\bm{I|z})p(\bm z)$ on human images. However, we adopt the belief that the hidden latent variable $\bm z$  depends \textit{only} on the appearance of the subject in the image $\bm I$. To achieve that, our encoder takes a pose independent human appearance $\bm T$ as input, and encodes it to part specific latent vectors $\bm z$. Furthermore, the encoded appearance $\bm z$ is warped by a target pose $P_t$ different than that of $I$, which is subsequently used by a generator.

%$\mathbb{E}_{I\sim p_{\text{data}}}[\int p(I, z) \,dz]$


%The encoding of our VAE is performed on the source appearance. However, the decoding of the VAE is performed on the warped latent code on the target pose to generate a photo realistic image. Our system is composed of fours steps.
%Our system performs encoding and decoding on different spaces in order to enforce cross pose appearance consistency and part based sampling capability. 

\subsection{The Proposed Approach}
We take pairs of images ($\bm{I_s}, \bm{I_t}$) of the same person (but in different poses) as input during the training. Our method is then described by four steps. 
In the first step,  we extract SMPL \textit{UV texture map} $\bm T_{s}$ from the input image $\bm I_s$  using the DensePose correspondences. In the second step, we use an encoding function $E$ to map the human appearance $\bm T_s$ of the source image to the parameters of the distribution of the latent vector. In the third step, we sample $\bm z$  from the estimated distribution of the source appearance. Given a target pose $\bm P_t$, we warp the encoded latent vector $\bm z$ to a noise image $\bm Z_t$ (Sec.~\ref{sec:warping}). In the forth step, we decode the warped noise image $\bm Z_t$ to a realistic image $\bm I_t'$ by a high fidelity generator network. Our method is summarized in Fig. \ref{fig:pipeline}.

%We take pairs of images ($\bm{I_s}, \bm{I_t}$) of the same person (but in different poses) as input during the training. Our method is described by four steps. 
%In the first step,  we extract SMPL \textit{UV texture map} $\bm T_{s}$ from the input image $\bm I_s$  using the Densepose correspondences (Sec. \ref{sec:texmap}). This encoding acts as a pose independent appearance of the subject in the input image. In the second step, we use an encoding function $E$ to map the human appearance $\bm T_s$ of the source image to the parameters of the distribution of the latent vector (Sec. \ref{sec:encoding}). In the third step, we sample $\bm z$  from the estimated distribution of the source appearance. Given a target pose $\bm P_t$, we warp the encoded latent vector $\bm z$ to a noise image $\bm Z_t$ (Sec. \ref{sec:warping}). In the forth step, we decode the warped noise image $\bm Z_t$ to a realistic image $\bm I_t'$ by a high fidelity generator network (Sec. \ref{sec:decoding}).

\paragraph{Extracting part-specific appearance}
\label{sec:texmap}
We use UV texture map of the SMPL surface model \cite{SMPL:2015} to represent appearance of the subject in the input image. 
%The normalized texture space provided by SMPL surface model \cite{SMPL:2015} is independent of the pose making it a good candidate for representing the appearance. 
The pixels of the input image $\bm{I_s}$ are transformed into UV space through mapping predicted by DensePose RCNN~\cite{Guler2018DensePose}. The pretrained network trained on COCO-DensePose dataset predicts  $24$ body segments and their part-specific \textit{U,V} coordinates of SMPL model. For easier mapping, the 24 part-specific UV maps are combined to form a single normalized UV texture map $\bm T_s$ in the format provided in SURREAL dataset \cite{varol17_surreal}. 
% 
This normalized (partial) texture map provides us with a pose-independent appearance encoding of the subject that is located spatially according to the body parts. The 24 regions in the texture map also provides us the placeholder for parts based noise sampling (see Sec.~\ref{sec:warping}), \textit{i.e.,} in our case, the number of body parts $M = 24$.  

\paragraph{Encoding part-specific appearance}
\label{sec:encoding}
As with VAE, we assume the distribution $q(\bm{z|T_s})$ of the latent code $\bm z$ given the appearance $\bm T_s$ to be Gaussian, $q(\bm{z|T_s}) \equiv \mathcal{N}(\bm{\mu_s, \sigma_s})$. We use a convolutional neural network $E(.)$ that takes the partial texture $\bm T_s$ as input and predicts the parameters ($\bm{\mu_s, \sigma_s}$) of the Gaussian distribution, $\bm{\mu_s, \sigma_s} \in \mathbb{R}^{M \times N}$.
The encoder comprises of a convolutional layer, 5 residual blocks, an average pooling layer, and finally a fully connected layer that produces the final output.
% The encoded appearance is then used to sample the noise vector subsequently warped and used by a decoder.

\paragraph{Warping latent space}
\label{sec:warping}
In the next step, we sample a latent code from the predicted distribution of the encoded appearance, $\bm z_s \sim E(\bm T_s) \equiv \mathcal{N}(\bm{\mu_s, \sigma_s})$. 
Given the  noise vector $\bm z_s$ and a target pose $\bm P_t$, 
we intend to reconstruct a realistic image $\bm \tilde I_t$ with the appearance encoded in  $\bm z_s \in \mathbb{R}^{M \times N}$ and pose from $\bm P_t$. We also want the latent code for a specific body part to have direct influence on the same body part in the generated image. We enforce this by warping and broadcasting the part based latent code to the corresponding part location in the target image and create a noise image $\bm Z_t \in \mathbb{R}^{H \times W \times N}$. Here, for each body part $k$, $\forall_{i,j \in k} \bm Z_t[i,j] \gets \bm z[k]$ (See the warping module in Fig. \ref{fig:pipeline}). This operation can be easily implemented by differentiable sampling given the DensePose image $P_t$. The design enables us to perform part based sampling during the test time. Other straightforward ways of using the noise vector, such as sampling noise in the UV texture space, tiling of a single noise vector in the entire spatial dimension, etc. did not give us the required result. See Sec.~\ref{sec:res:appearance} and \ref{sec:res:parts}  for a detailed analysis.


\paragraph{Decoding to a Photo-Realistic image}
\label{sec:decoding}
The warped noise image in the target pose $\bm Z_t$ with the noise vectors correctly aligned with the body parts in the target pose, is used as an input to a generator network $G(.)$. The generator along with the warping module acts as the conditional decoder of our pipeline. We use the high fidelity generator from Pix2PixHD \cite{wang2018pix2pixHD} that comprises of a 3 down-sampling blocks, 6   residual blocks and a 3 up-sampling blocks for this purpose.

%Note that, we are encoding the appearance 

%The discriminator for adversarial training of RenderNet also uses the multiscale design of Pix2PixHD . In our experiments, we use a three scale discriminator network for adversarial training. 


\subsection{Training Details}
\label{sec:training}
%During the training, our system takes source-target pairs images ($\bm{I_s}, \bm{I_t}$) of the same person in different poses. The corresponding poses ($\bm{P_s}, \bm{P_t}$) is directly computed from the input images by a pretrained DensePose RCNN. The appearance in the form of UV texture map $\bm T_s$ is then extracted from the source image and passed through the encoder $E(.)$. The sampled noise $\bm z_s$ from the encoder is warped as $\bm Z_t$ using the target pose $\bm{P_t}$, and passed through the translation network $G(.)$ that acts as a decoder.
%Our system performs encoding in the normalized texture space, but it performs decoding in the target pose space. 
Our entire training pipeline can be summarized by the following equations.

\begin{equation}\label{eq:sampling}
  \begin{aligned}
\bm z_s \sim E(\bm T_s), \qquad \bm{\tilde I_{t}} = G(\bm Z_t),\\
 \end{aligned}
\end{equation}

where $\bm Z_t = W(\bm z_s, \bm P_t)$ and $W(.)$  the differentiable warping function as described in Sec.~\ref{sec:warping}.
With the re-parameterization trick \cite{Kingma2014VAE} for sampling $z_s$, the entire pipeline becomes differentiable allowing direct back-propagation to the parameters of $E(.)$ and $G(.)$. The pipeline is trained with an objective $\mathcal{L}_{total}$ derived from Conditional VAE-GAN:

\begin{equation}\label{eq:loss}
 \mathcal{L} =  \mathcal{L}_{rec} +  \mathcal{L}_{GAN} +  \mathcal{L}_{prior}
\end{equation}

The three loss terms, $\mathcal{L}_{rec}, \mathcal{L}_{GAN}$ and $\mathcal{L}_{prior}$ are described below.

\vspace{-0.3cm}
\paragraph{Reconstruction Loss}:
The reconstruction loss $\mathcal{L}_{rec}= \lambda_{VGG} L_{VGG} + \lambda_{face}L_{face}$ quantifies the dissimilarity between generated image $\bm {\tilde I_t}$ and the ground truth image $\bm I_t$. It comprises of the following terms.
\vspace{-0.2cm}
\begin{itemize}[leftmargin=*]
\itemsep-0.2em
\item \textit{Perceptual Loss}: We use perceptual loss, which is the difference between the activations on different layers of the pre-trained VGG network \cite{simonyan2014very} applied on the generated image and the ground truth image.
$L_{VGG} = \sum \frac{1}{N^j}|l^j(\bm {\tilde I_t}) - l^j(\bm I_t)|_1$.
% 
Here, $l^j$ is the activation and $N^j$ the number of elements of the j-th layer in the ImageNet pre-trained VGG network. 

\item \textit{Face Identity Loss} To better preserve facial identity, we use a pre-trained network SphereFaceNet \cite{liu2017sphereface} $S_{face}(.)$ on the cropped 
face of the generated image and the ground truth image, $L_{face} = |S_{face}(\bm I_{t}) - S_{face}(\bm {\tilde I_t})|_1.$
\end{itemize}

%The total reconstruction loss is then $$\mathcal{L}_{rec}= \lambda_{VGG} L_{VGG} + \lambda_{face}L_{face}.$$
\vspace{-0.3cm}
\paragraph{GAN Loss -- $\mathcal{L}_{GAN}$}: The GAN loss $\mathcal{L}_{GAN}= \lambda_{D} L_D + \lambda_{FM}L_{FM}$ pushes the generator to generate realistic images. We use the multiscale discriminator architecture $D$ from Pix2PixHD \cite{wang2018pix2pixHD} for implementing the GAN loss. The network $D$ is conditioned on both the generated image and warped noise image at different scales. The total GAN loss  comprises of the following terms.
\vspace{-0.2cm}
\begin{itemize}[leftmargin=*]
\itemsep-0.2em
\item \textit{Multiscale adversarial loss} We use 2 scale discriminator the adversarial loss $L_D$. 
%$D = (D_1, D_2, D_3)$ operating on different scales.
%
%$$ \mathcal{L}_{D} = \operatorname*{min}\limits_{G} \operatorname*{min}\limits_{D_1, D_2, D_3} \sum_{i = 1, 2, 3} L_{GAN}(G, D_i)$$
\item \textit{Discriminator FM loss}: We use a discriminator feature matching $L_{FM}$, which is the difference between the activations on the different layers of the discriminator applied on the generated image and the real image.
%$$\mathcal{L}_{GAN}= \lambda_{D} L_D + \lambda_{FM}L_{FM}.$$
\end{itemize}

Please refer to \cite{wang2018pix2pixHD} for more details on the adversarial loss with multiscale discriminator. 
%\KS{Describe the losses by exact formulas if you have space before the submission}.

\vspace{-0.3cm}
\paragraph{Prior loss -- $\mathcal{L}_{prior}$}:
To enable sampling at inference time, the encoding $E(\bm T_s)$ is encouraged to be close to a standard Gaussian distribution, \textit{i.e.,} the prior distribution on the $z$ vector is assumed to be $\mathcal{N}(0, I)$. Therefore, we employ the prior loss 
$\mathcal{L}_{prior} = \lambda_{KL} \mathcal{D}_{KL}(E(\bm T_s)||\mathcal{N}(0, I)),$
where $\mathcal{D}_{KL}(p||q)$ is the Kullback-Leibler divergence between the probability distributions $p(x)$ and $q(x)$. 

With re parameterization trick on sampling $\bm z_s$, we train the system end-to-end and optimize the parameters of the network $E, G$ and $D$. The final objective $\mathcal{L}_{total}$ in Eq. \ref{eq:loss} is minimized with respect to the generator $G$ and the encoder $E$, while maximized with respect to the the discriminator $D$.
We use Adam optimiser \cite{adam} for our optimization with an initial learning rate of 2$\times 10^4$, $\beta_1$ as 0.5 and no weight decay. The loss weights are set empirically to $\lambda_{VGG} = 10, \lambda_{face} = 5, \lambda_{D} = 1, \lambda_{FM} = 10, \lambda_{KL} = 0.01$. For speed, we pre-compute DensePose on the images and directly read them as input.

\begin{figure*}[t] 
    \includegraphics[width=\linewidth]{Figures/appearance_qual.jpg} 
    \caption{Result of our method for pose guided image generation, and its comparision with VUNet \cite{esser2018variational} and other baselines. The conditioning pose is shown in the left corner. Our approach produces samples of high quality than the baseline methods.} 
    \label{fig:appearance} 
\end{figure*} 


\subsection{Testing - sampling across pose and body parts}

During testing, we sample the appearance vector $\bm z$ from the prior distribution. We warp $\bm z$ with the conditioning pose $P$ and feed the resulting noise image to the trained generator $G$ to get a generated image $\bm I_{z,P}$. 

\begin{equation}\label{eq:sampling}
  \begin{aligned}
\bm z \sim \mathcal{N}(0, I), \qquad \bm{I_{z,P}} = G(\bm Z_P),\\
 \end{aligned}
\end{equation}

where $\bm Z_P = W(\bm z_, \bm P)$; $W(.)$  the warping function. The appearance $\bm z$ can be also encoded from an input image by using the encoder on its partial texture map  $\bm T$, \textit{i.e.,} $\bm z = \bm \mu$ where $\bm \mu, \bm \sigma = E(\bm T)$. Keeping $\bm z$ fixed and varying the the pose $\bm P$, we can perform pose transfer \cite{Sarkar2020,Grigorev2019CoordinateBasedTI,Siarohin2019AppearanceAP,Neverova2018} -- re-rendering a subject with different pose and viewpoint. We can also perform body parts based sampling by only varying the vector $\bm z[k]$ corresponding to the part $k$. See Sec.~\ref{sec:results} for all possible applications of our system.




==> HumanGan_ A Generative Model of Humans - arxiv/Sections/method_new.tex <==
%!TEX root = ../cvpr.tex
 


\section{Method}
\label{sec:method}


Our goal is to learn a generative model of human images, which is conditioned on body pose and a low dimensional latent vector encapsulating the appearance of different body parts. 
%
We use DensePose~\cite{Guler2018DensePose} to represent the human pose. Our task can be then formulated as a deterministic mapping $G:(\bm P, \bm z) \rightarrow \bm I$. Here, $\bm P \in \mathbb{R}^{H \times W \times 3}$ is a three-channel DensePose image representing the conditioning pose, $\bm z \in \mathbb{R}^{M \times N}$ is the latent vector comprised of $M$ human body parts and $N$ part-specific latent vector dimensions, and $\bm I \in \mathbb{R}^{H \times W \times 3}$ is the generated image. 


%For learning such function with a latent variable capturing the ambiguous aspect of the output, we build our method on Variational Auto-Encoder (VAE) \cite{Kingma2014VAE}. 
For learning such function, we build our method on variational autoencoders (VAE) \cite{Kingma2014VAE}. 
As in any latent vector model, the observed variable of images $\bm I$ is assumed to be dependent on the unobserved hidden latent variable $\bm z$ that encodes semantically meaningful information about $\bm I$.  The goal is then to find their joint distribution $p(\bm{I, z})$ by maximizing the evidence lower bound (ELBO) -- by jointly optimizing the encoder $q(\bm{z|I})$ and the decoder $p(\bm{I|z})$.
In this work, our \textit{key assumption} is that the latent variable $\bm z$  depends \textit{only} on the appearance of the subject in the image $\bm I$. To enforce that, we first extract a pose-independent human appearance $\bm T$ from $\bm I$. Our encoder $q(\bm{z|T})$ is then conditioned on $\bm T$ (which is actually a function of $\bm I$), to encode to part-specific latent vector $\bm z$. 
% 
Furthermore, the encoded appearance $\bm z$ is warped by a target pose $\bm P_t$ different from the pose in $\bm I$, which is subsequently used by a generator. 
% Our method is concretely described in the following subsection. 
We next describe our method in detail. 
% 


\subsection{Our Architecture} 
% 
In the training stage, we take pairs of images ($\bm{I_s}, \bm{I_t}$) of the same person (but in different poses) as input. Our method performs in four steps. 
In the first step,  we extract SMPL \textit{UV texture map} $\bm T_{s}$ from the input image $\bm I_s$  using the DensePose correspondences. In the second step, we use an encoding function $E$ to map the human appearance $\bm T_s$ of the source image to the parameters of the distribution of the latent vector. In the third step, we sample $\bm z$  from the estimated distribution of the source appearance. Given a target pose $\bm P_t$, we warp the encoded latent vector $\bm z$ to a noise image $\bm Z_t$. In the fourth step, we decode the warped $\bm Z_t$ to a realistic image $\bm I_t'$ by a high-fidelity generator network. Our method is summarized in Fig.~\ref{fig:pipeline}. 
 
\noindent\textbf{Extracting Appearance.} 
\label{sec:texmap}
We use a UV texture map of the SMPL surface model \cite{SMPL:2015} to represent the subject's appearance in the input image. 
%The normalized texture space provided by SMPL surface model \cite{SMPL:2015} is independent of the pose making it a good candidate for representing the appearance. 
The pixels of the input image $\bm{I_s}$ are transformed into the UV space through a mapping predicted by DensePose RCNN~\cite{Guler2018DensePose}. The pretrained network trained on COCO-DensePose dataset predicts  $24$ body segments and their part-specific \textit{U,V} coordinates of SMPL model. For easier mapping, the 24 part-specific UV maps are combined to form a single normalized UV texture map $\bm T_s$ in the format provided in SURREAL dataset \cite{varol17_surreal}. This normalized (partial) texture map provides us with a pose-independent appearance encoding of the subject that is located spatially according to the body parts. The 24 part segments in the texture map also provide us the placeholder for part-based noise sampling, \textit{i.e.,} in our case, the number of body parts $M = 24$. 

\noindent\textbf{Encoding Appearance.} 
\label{sec:encoding}
As with VAE, we assume the distribution $q(\bm{z|T_s})$ of the latent code $\bm z$, given the appearance $\bm T_s$ to be Gaussian, $q(\bm{z|T_s}) \equiv \mathcal{N}(\bm{\mu_s, \sigma_s})$. We use a convolutional neural network $E(\cdot)$ that takes the partial texture $\bm T_s$ as input and predicts the parameters ($\bm{\mu_s, \sigma_s}$) of the Gaussian distribution, $\bm{\mu_s, \sigma_s} \in \mathbb{R}^{M \times N}$. 
% 
The encoder comprises a convolutional layer, five residual blocks, an average pooling layer, and finally, a fully connected layer that produces the final output.
% The encoded appearance is then used to sample the noise vector subsequently warped and used by a decoder.

\noindent\textbf{Warping Latent Space.} 
\label{sec:warping} 
In the next step, we sample a latent code from the predicted distribution of the encoded appearance, $\bm z_s \sim E(\bm T_s) \equiv \mathcal{N}(\bm{\mu_s, \sigma_s})$. 
Given the noise vector $\bm z_s$ and a target pose $\bm P_t$, 
we intend to reconstruct a realistic image $\bm I_t'$
with the appearance encoded in  $\bm z_s \in \mathbb{R}^{M \times N}$ and pose from $\bm P_t$. We also want the latent code for a specific body part to have direct influence on the same body part in the generated image. 
% 
We enforce this by warping and broadcasting the part-based latent code to the corresponding part location in the target image and create a noise image $\bm Z_t \in \mathbb{R}^{H \times W \times N}$. Here, for each body part $k$, $\forall_{i,j \in k} \bm Z_t[i,j] \gets \bm z[k]$ (see the warping module in Fig.~\ref{fig:pipeline}). 
% 
This operation can be easily implemented by differentiable sampling $W(\cdot)$ given the DensePose image $\bm P_t$, \textit{i.e.} $\bm Z_t = W(\bm z_s, \bm P_t)$. The design enables us to perform part-based sampling during the test time. 
% 
Other straightforward ways of using $\bm z_s$, such as sampling noise in the UV texture space or tiling of a single noise vector in the entire spatial dimension, did not give us the required result. 
% 
See Sec.~\ref{sec:res:appearance} and \ref{sec:res:parts} for a detailed analysis.


\noindent\textbf{Decoding to a Photo-Realistic Image.} 
\label{sec:decoding}
The warped noise image in the target pose $\bm Z_t$ with the noise vectors correctly aligned with the body parts in the target pose, is used as an input to a generator network $G(\cdot)$. 
%
% 
The generator and the warping module act as the conditional decoder of our pipeline. 
% 
We use the high-fidelity generator from Pix2PixHD \cite{wang2018pix2pixHD} that comprises three down-sampling blocks, six residual blocks and three up-sampling blocks. 
% 
%Note that, we are encoding the appearance 

%The discriminator for adversarial training of RenderNet also uses the multiscale design of Pix2PixHD . In our experiments, we use a three scale discriminator network for adversarial training. 


\subsection{Training Details}
\label{sec:training}

Our entire training pipeline can be summarized by the following equations: 
% 
\begin{equation}\label{eq:sampling}
  \begin{aligned}
\bm z_s \sim E(\bm T_s), \quad \bm Z_t = W(\bm z_s, \bm P_t), \quad \bm{ I_{t}'} = G(\bm Z_t),\\
 \end{aligned}
\end{equation}
% 

With the re-parameterization trick \cite{Kingma2014VAE} for sampling $\bm z_s$, the entire pipeline becomes differentiable, allowing direct back-propagation to the parameters of $E(\cdot)$ and $G(\cdot)$. The pipeline is trained with an objective $\mathcal{L}_{total}$ derived from conditional VAE-GAN: 
% 
\begin{equation}\label{eq:loss}
 \mathcal{L}_{total} =  \mathcal{L}_{rec} +  \mathcal{L}_{GAN} +  \mathcal{L}_{prior}. 
\end{equation}
% 
We describe in the following all three loss terms of \eqref{eq:loss}. 
% 

\noindent\textbf{Reconstruction Loss.} 
% 
The reconstruction loss $\mathcal{L}_{rec}= \lambda_{VGG} L_{VGG} + \lambda_{face}L_{face}$ quantifies the dissimilarity between the generated image $\bm {\tilde I_t}$ and the ground-truth image $\bm I_t$. 
% 
It comprises 1) \textit{Perceptual Loss $L_{VGG}$} which is the difference between the activations on different layers of the pre-trained VGG network \cite{simonyan2014very} applied on the generated image and the ground-truth image; 
%
and
%
2) \textit{Face Identity Loss $L_{face}$}  which is the difference between features of the pre-trained SphereFaceNet \cite{liu2017sphereface} on the cropped 
face of the generated image and the ground-truth image.
%$L_{face} = |S_{face}(\bm I_{t}) - S_{face}(\bm {\tilde I_t})|_1.$






%The total reconstruction loss is then $$\mathcal{L}_{rec}= \lambda_{VGG} L_{VGG} + \lambda_{face}L_{face}.$$
% \vspace{-0.3cm}
\noindent\textbf{GAN Loss.} The GAN loss $\mathcal{L}_{GAN}= \lambda_{D} L_D + \lambda_{FM}L_{FM}$ pushes the generator to generate realistic images. We directly use the two-scale discriminator architecture $D$ from Pix2PixHD \cite{wang2018pix2pixHD} for implementing the GAN loss. The network $D$ is conditioned on both generated image and warped noise image at different scales. The total GAN loss  comprises of multiscale adversarial loss $L_D$ and discriminator feature matching loss $L_{FM}$. 
% 
See \cite{wang2018pix2pixHD} for more details. 



% \vspace{-0.3cm}
\noindent\textbf{Prior Loss $\mathcal{L}_{prior}$.} 
% 
To enable sampling at inference time, the encoding $E(\bm T_s)$ is encouraged to be close to a standard Gaussian distribution, \textit{i.e.,} the prior distribution on the $\bm z$ 
vector is assumed to be $\mathcal{N}(0, I)$. Therefore, we employ the prior loss 
$\mathcal{L}_{prior} = \lambda_{KL} \mathcal{D}_{KL}(E(\bm T_s)||\mathcal{N}(0, I)),$
where $\mathcal{D}_{KL}(p||q)$ is the Kullback-Leibler divergence between the probability distributions $p(x)$ and $q(x)$. 

With reparameterization trick on sampling $\bm z_s$, we train the system end-to-end and optimize the parameters of the networks $E, G$ and $D$. The final objective $\mathcal{L}_{total}$ in Eq.~\eqref{eq:loss} is minimized with respect to the generator $G$ and the encoder $E$, while maximized with respect to the the discriminator $D$.
We use Adam optimiser \cite{adam} for our optimization with an initial learning rate of 2$\times 10^{-4}$, $\beta_1$ as 0.5 and no weight decay. The loss weights are set empirically to $\lambda_{VGG} = 10, \lambda_{face} = 5, \lambda_{D} = 1, \lambda_{FM} = 10, \lambda_{KL} = 0.01$. For speed, we pre-compute DensePose on the images and directly read them as input.

\begin{figure*}[t] 
    \includegraphics[width=\linewidth]{Figures/appearance_qual.jpg} 
    \caption{Results of our HumanGAN approach for pose-guided image generation, and its comparison with VUNet \cite{esser2018variational}, Pix2PixHD+Noise, Pix2PixHD+WNoise and Deterministic Auto Encoder (DAE). The conditioning pose is shown in the left corner. Our approach produces samples of higher quality than the baseline methods.} 
    \label{fig:appearance} 
\end{figure*} 



\subsection{Inference: Sampling Poses and Body Parts} 

During testing, we \textit{sample} the \textit{appearance} vector $\bm z$ from the prior distribution. We warp $\bm z$ with the conditioning pose $\bm P$ and feed the resulting noise image to the trained generator $G$ to get a generated image $\bm I_{z,P}$: 
% 
\begin{equation}\label{eq:sampling}
  \begin{aligned}
\bm z \sim \mathcal{N}(0, I),  \quad \bm Z_P = W(\bm z, \bm P), \quad \bm{I_{z,P}} = G(\bm Z_P),\\
 \end{aligned}
\end{equation}
% 


% 
The appearance $\bm z$ can also be encoded from an input image by using the encoder on its partial texture map  $\bm T$, \textit{i.e.,} $\bm z = \bm \mu$, where $\bm \mu, \bm \sigma = E(\bm T)$. Keeping $\bm z$ fixed and varying the the pose $\bm P$, we can perform \textit{pose transfer} \cite{Sarkar2020,Grigorev2019CoordinateBasedTI,Siarohin2019AppearanceAP,Neverova2018}, \textit{i.e.,} re-rendering a subject with  different pose and viewpoint. 
% 
We can also perform \textit{parts-based sampling} and \textit{garment transfer} by only varying the vector $\bm z[k]$ corresponding to the part $k$.
% 
See Sec.~\ref{sec:results} for all possible  applications of our system. 
% 









==> HumanGan_ A Generative Model of Humans - arxiv/Sections/related_work.tex <==
%!TEX root = ../cvpr.tex

\section{Related Work}

\noindent\textbf{Deep Gernerative Models} have made remarkable achievements on image generation. 
As the original GAN model~\cite{Goodfellow14} was only able to synthesize low-resolution images, % with limited quality. 
the follow-ups improved it with multiple % the synthesis 
discriminators~\cite{GMAN,Mordido2018DropoutGANLF,Doan2019OnlineAC}, self-attention  mechanism~\cite{sagan,Brock2018Biggan} and progressive training  strategy~\cite{karras2018progressive}. 
These methods use a single latent vector $\mathbf{z}$ to resemble the latent factor distribution of training data, which leads to unavoidable entanglements  and limited control over image synthesis. 
% 
StyleGANs~\cite{karras2019style, Karras2019stylegan2} 
% and StyleGAN2 
approach this problem by mapping $\mathbf{z}$ to an intermediate latent space $\mathbf{w}$, which is then fed into the generator to change different levels of attributes. 
% 
Although it enables 
% Although the StyleGAN family has 
more control on image synthesis, it does not disentangle different feature factors. 
Recent works~\cite{tewari2020stylerig,tewari2020pie} extend StyleGAN to synthesize images of faces with a rig-like control over 3D interpretable face parameters such as face pose, expression and scene illumination. 
% 
Compared to faces, synthesizing the full human appearance with control of 3D body pose and human appearance is a much more difficult problem due to more severe 3D pose and appearance changes. 
% 
We propose the first method to this problem allowing photo-realistic image synthesis of a full human body with controls of the 3D pose as well as the appearance of each body part. % 

\noindent\textbf{Conditional GAN} 
(cGAN) % is a type of GAN 
uses conditional information for the generator and discriminator. cGAN is useful for applications such as class conditional image generation~\cite{mirza2014conditional,miyato2018cgans,pmlr-v70-odena17a} and image-to-image translation~\cite{pix2pix2017,wang2018pix2pixHD}.
Many works~\cite{mirza2014conditional,pix2pix2017,wang2018pix2pixHD,park2019SPADE,wang2018vid2vid} require paired data for fully-supervised training. 
% 
Pix2Pix~\cite{pix2pix2017} and Pix2PixHD~\cite{wang2018pix2pixHD} learn the mapping from input images to output images. 
Some works~\cite{CycleGAN2017,YiZTG2017,LiuBK2017,choi2017stargan,Recycle-GAN} tackle a harder problem of learning the mapping between two domains based on unpaired data. 
cGAN is a deterministic model which produces a single output. 
% 
Our approach also applies a conditional GAN to map from a warped noise image to output images. 
% 
However, unlike cGAN methods, we are able to randomly sample noise from a normal distribution for each body part for synthesizing different output images. 




\begin{figure*}[t] 
    \includegraphics[width=\linewidth]{Figures/pipeline2.png} 
    \caption{\textbf{Overview of our method.} Given a source image $\bm I_s$, we extract a UV texture map of the human appearance $\bm T_s$. 
    % 
    The encoder then encodes $\bm T_s$ to part-specific latent vectors $\bm z_s$. 
    % 
    The target pose $\bm P_t$ is used to warp and broadcast the latent vectors to the corresponding parts in the target image to create a noise image $\bm Z_t$.
    % 
    Finally, the generator converts $\bm Z_t$ to a realistic image. 
    % 
    At testing, we generate random samples by controlling the latent vectors $\bf z \in \mathcal{N}(0,1)$ and the target pose $\bm P_t$.
    %
    } 
    \label{fig:pipeline} 
    \vspace{-0.5cm}
\end{figure*}


\noindent\textbf{Pose Transfer} % \KS{Reduce this section for space} 
% 
% \emph{Pose transfer} 
refers to the problem of transferring person appearance from one pose to another \cite{MaSJSTV2017}. 
% 
Most approaches formulate it as an image-to-image mapping problem, \textit{i.e.,} given a reference image of target person, mapping the body pose in the format of renderings of a  skeleton~\cite{chan2019dance,SiaroSLS2017,Pumarola_2018_CVPR,KratzHPV2017,zhu2019progressive}, dense  mesh~\cite{Liu2019,wang2018vid2vid,liu2020NeuralHumanRendering,Sarkar2020,Neverova2018,Grigorev2019CoordinateBasedTI}, dense labeled pose maps \cite{Yoon2021} or joint position  heatmaps~\cite{MaSJSTV2017,Lischinski2018,Ma18} to real images. 
% 
% 
Though our method is not specifically designed for pose transfer, it can also be applied to this problem with high-quality results, as our generated samples retain identity across different poses. We demonstrate this in Sec.~\ref{sec:results}. 



\noindent\textbf{Variational Autoencoders} % as Generative Model 
 (VAE) are likelihood-based models which can effectively model stochasticity \cite{Kingma2014VAE}. 
% 
Larsen \textit{et al.}~\cite{larsen2016autoencoding} first introduced a combined VAE and GAN to achieve higher quality than vanilla VAE. 
% 
VUNet~\cite{esser2018variational} combined VAE with UNet for pose-guided image generation. 
% 
Lassner \textit{et al.}~\cite{Lassner2017} present a two-stage VAE framework 
% where they, rendered 
using a parametric model of human meshes \cite{SMPL:2015} as pose and shape conditioners. 
% 
Our method builds on conditional VAE-GAN. 
% 
Unlike the existing methods, it generates images of higher resolution and quality, and offers more control over part sampling and garment transfer. 
% 



==> HumanGan_ A Generative Model of Humans - arxiv/Sections/results.tex <==
%!TEX root = ../cvpr.tex

\section{Experimental Results} 
\label{sec:results}

\noindent\textbf{Dataset.} 
% 
We use the \textit{In-shop Clothes Retrieval Benchmark} of DeepFashion dataset \cite{Liu2016DeepFashion} for our main experiments. 
% 
The dataset comprises of around 52K high-resolution images of fashion models with 13K different clothing items in different poses. Training and testing splits are also provided. To filter non-human images, we discard all the images where we could not compute DensePose, resulting in 38K training images and 3K testing images. We train our system with the resulting training split and use the testing split for conditioning poses. We also show qualitative results of our method with Fashion dataset \cite{Zablotskaia2019DwNetDW} that has 500 training and 100 test videos, each containing roughly 350 frames. 


\noindent\textbf{Experimental Setup.} 
% 
We train our model for the resolution of 512 $\times$ 512 with the training procedure described in Sec.~\ref{sec:training}. The resolution of the partial texture map $T$ is chosen to be 256 $\times$ 256, number of body parts $M = 24$, and the latent vector dimension $N = 16$. To evaluate our model for the ability to generate diverse and realistic images, preserve the identity of the generated output across different poses, and perform part-based sampling, we use the \textit{same trained model} for \textit{all the experiments} in the following subsections. 
% 
All the ablation experiments use the same setting in terms of output resolution. When the result of the comparison methods do not have a trained model for 512 resolution (especially for the SOA methods on pose transfer), we resize our image before performing the quantitative evaluation. 


\begin{figure*}[t]
    % \includegraphics[width=\linewidth]{Figures/SOA.pdf} 
    \includegraphics[width=\linewidth]{Figures/appearance_latent.jpg}
    \caption{Generated images with interpolated appearance encodings. Note that each of the intermediate images is a coherently dressed human image. 
    % The conditioning pose is not shown.
    } 
    \label{fig:latent_inter} 
\end{figure*}
\subsection{Appearance Sampling} 
\label{sec:res:appearance}
We next evaluate the ability of our system to generate diverse and realistic images of humans given a conditioning pose. Given a \textit{fixed pose}, we \textit{randomly generate samples} from the latent vector $\bm z \sim \mathcal{N}(0^{MN}, I^{MN})$ and compare our method with the following baseline methods. 

\begin{table}[t]
\small
\centering
\begin{tabular}{c|c|c} 
              & \textbf{Diversity}    & \textbf{Realism}   \\ 
              &LPIPS Distance $\uparrow$& FID $\downarrow$\\\hline
VUnet  \cite{esser2018variational}           &   0.182      &     50.0  \\              
Pix2PixHD+Noise          &  4.6e-6    &   109.4    \\
Pix2PixHD+WNoise          &  0.008        &   101.9    \\
DAE+WNoise        &  0.083      &   187.4   \\
\textbf{Ours} & \textbf{0.219}  &  \textbf{24.9}   \\ \hline
ground truth  & 0.44 &  0.0  \\ 
\end{tabular}
\caption{Diversity \textit{vs} realism. We use LPIPS distance \cite{zhang2018perceptual} between the randomly generated samples of the same pose to measure Diversity, and FID to measure the realism of the generated samples. $\uparrow$ ($\downarrow$) means higher (lower) is better.} 
\label{table:appearance}
\vspace{-0.3cm}
\end{table}



\noindent\textbf{Pix2PixHD + Noise.} %Conditional image
% 
Some generators, such as Pix2Pix, Pix2PixHD produces a single output given a conditional input. 
Randomly drawn noise from a prior distribution can be added to the input of conditional generators to induce stochasticity. We sample noise $z \in \mathbb{R}^N$ from the standard Gaussian distribution and tile it across the 3 channel condition DensePose image to produce $3+N$ channel input vector and train Pix2PixHD for a pose-conditioned multimodal human generator. 
%\textit{i.e.} we perform the following optimization on the conditional generator $G$ and discriminator $D$: 
We optimize the conditional generator $G$ and discriminator $D$ with the GAN loss:
$\max\limits_{D}\min\limits_{G} \mathbb{E}_{\bm{P,T} \sim p(\bm{P,T)}}[\log(D(\bm{P,I}))] + \mathbb{E}_{\bm P\sim p(\bm P), \bm z \sim p(\bm z)}[\log(1-D(\bm P, G(\bm P, \bm z))]$, and the reconstruction loss between $G(\bm P, \bm z)$ and $\bm I$.

\noindent\textbf{Pix2PixHD + Warped Noise.} 
% 
Isola \textit{et al.}~\cite{pix2pix2017} and Zhu \textit{et al.}~\cite{NIPS2017_6650} observed that a simple extension of a translation network with noise for the purpose multimodal generation often ends up in mode collapse. Therefore, we extend our \textit{Pix2PixHD + Noise} baseline by sampling part specific noise vector $\bm z \in \mathbb{R}^{M \times N}$ and warping it with the input DensePose to create a noise image $\bm Z_P$ as in Sec.~\ref{sec:warping}. This noise image is used as conditioning input to Pix2PixHD. 
% 

\noindent\textbf{Deterministic Auto Encoder with Warped Noise (DAE).} 
% 
This baseline serves as the deterministic version of our method. Because of the lack of constraints on the latent variable (KL divergence with the prior), and direct broadcasting of a single noise vector to multiple pixels in the warping operation, we encountered the problem of exploding gradients. To make the training process tractable, we use a UNet to encode the appearance to the UV texture space, $\bm Z_s = E(\bm T_s), \bm Z_s \in \mathbb{R}^{h \times w \times N}$ ($h, w$ are the texture map dimensions). 
% 
We warp $\bm Z_s$ from the texture coordinates to the pixel coordinates by the target pose (instead of a single vector per parts) to complete the pipeline for training. 
% 
Because of the similarity of this baseline to NHRR~\cite{Sarkar2020}, we use UNet configuration as in their work. 

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Figures/transfer_small.png}
    \caption{% Pose Transfer -- 
    Comparison of our reconstruction+transfer results with the state-of-the-art pose transfer methods: CBI \cite{Grigorev2019CoordinateBasedTI},  NHRR \cite{Sarkar2020},  DSC \cite{Siarohin2019AppearanceAP}, VUNet \cite{esser2018variational}, and DPT. Our approach produces more realistic renderings than the competing methods. Best viewed when zoomed digitally. More results are provided in the appendix.} 
    \label{fig:transfer} 
    \vspace{-0.3cm}
\end{figure}



\begin{table}[t] 
\resizebox{\columnwidth}{!}{% 
\centering 
\begin{tabular}{@{}c|c|c||c|c|c@{}} 
              & SSIM $\uparrow$   & LPIPS  $\downarrow$ & & SSIM $\uparrow$   & LPIPS  $\downarrow$ \\ \hline
CBI  \cite{Grigorev2019CoordinateBasedTI}          &  0.766     &   0.178 &DPT \cite{Neverova2018}           &   0.759      &     0.206     \\
DSC \cite{Siarohin2019AppearanceAP}          &  0.750        &   0.214     & NHRR \cite{Sarkar2020} & {0.768}  &  \textbf{0.164}   \\ 
VUNet  \cite{esser2018variational}       &  0.739      &    0.202  & \textbf{Ours} & \textbf{0.777}  &  {0.187}  \\ \hline
%GT  & 1.0 &  0.0   \\ 
\end{tabular}} 
\caption{Quantitative results for pose transfer against several  state-of-the-art methods using Structural Similarity Index (SSIM) \cite{ssim2004} and Learned Perceptual Image Patch Similarity (LPIPS)  \cite{zhang2018perceptual}. $\uparrow$ ($\downarrow$) means higher (lower) is better.} 
\label{table:transfer} 
\vspace{-0.4cm} 
\end{table} 

\noindent\textbf{VUNet \cite{esser2018variational}.} 
% 
We compare our result to VUNet that performs disentanglement between appearance and structure and can be used for human generation. We use their publically available code and trained model on DeepFashion dataset and report their results here. Note that in contrast to our  method, VUNet cannot perform part-based sampling  (Sec.~\ref{sec:res:parts}). 

\noindent\textbf{Additional Baselines} We perform following additional baselines during development and training of our model: a) \textit{NoParts} does not perform part-specific warping, but broadcasts concatenated part-encoded noise-vector to the human silhouette (see Sec. \ref{sec:res:parts} for more details on this) 
%b) \textit{NoWarp-DPCond} broadcasts the noise vector to each pixel and directly condition the DensePose image to the decoder. 
b) \textit{+DPCond} conditions the DensePose image $\bm P_t$ in addition to the noise image $\bm Z_t$ to the generator. c) \textit{+NoisePrior} use samples from the prior $\mathcal{N}(0,1)$  (along with the encoded distribution) during the training, as recommended by Larsen \textit{et al.}~\cite{larsen2016autoencoding}. All the aforementioned \textit{additional baselines} performed poorly, and we present their results in the appendix. We discuss here the main baselines that are most representative of the different methods.
\begin{figure*}[t]
    % \includegraphics[width=\linewidth]{Figures/SOA.pdf} 
    \includegraphics[width=\linewidth]{Figures/part_sampling_2.jpg}
    \caption{Our results for part sampling. 
    % 
    We change the latent noise corresponding to a specific body part. 
    % , we can perform part sampling.
    % 
    } 
    \label{fig:parts} 
\end{figure*}
\begin{figure}[t]
    % \includegraphics[width=\linewidth]{Figures/SOA.pdf} 
    \includegraphics[width=\linewidth]{Figures/fashion.png} 
    \caption{Results of our method for motion transfer in a walking  sequence from fashion dataset \cite{Zablotskaia2019DwNetDW}. See the accompanying video for the motion results.
    % The conditioning target poses are not shown. 
    } 
    \label{fig:fashion} 
    \vspace{-0.5cm}
\end{figure}

The qualitative results are shown in Fig.~\ref{fig:appearance}. 
% 
We find that \textit{Pix2PixHD+N} produces a single realistic output on the conditioning pose and undergo full mode collapse. The baseline \textit{Pix2PixHD+WN} produces slightly diverse output than \textit{Pix2PixHD+N}, but the variations are still not meaningful. While the deterministic method of \textit{DAE} is a right choice for reconstruction and pose transfer (see results of NHRR \cite{Sarkar2020} in Sec.~\ref{sec:res:posetransfer}), 
there is no guarantee that the distribution of the encoded latent space will be close to a prior distribution, which makes the test-time sampling difficult. This makes the output far from realistic when the latent vector is sampled from  $\mathcal{N}(0, I)$. VUNet produces a diverse output  but lacks the quality due to its less powerful generator. In contrast, we find that our full method produces results that are both diverse and realistic. We also find our latent space of appearance to be smooth and interpolateable. Fig.~\ref{fig:latent_inter} shows images generated by interpolating the appearance vector $\bm z$ between two encodings. Note how each of the intermediate images is a coherently dressed human image. More qualitative results are provided in the appendix. 
% 

% 
To evaluate our method quantitatively, we randomly select 100 poses from the test set and generate 50 samples for each pose for all the methods. We measure diversity and realism of all the baselines by the following metrics \textit{1) Pairwise LPIPS distance} -- we compute LPIPS distance \cite{zhang2018perceptual} between all the generated samples for each pose, and take the mean of the distances of all such pairs. More the value of this metric, more diverse is the output. \textit{2) FID}-- we compute the Frech{\^e}t Inception Distance between the generated samples and the training split of the dataset. FID captures how close is the distribution of the generated samples, from the distribution of the ground truth in the InceptionV3 feature space, and it has been used widely in the community as a metric for quality for GANs  \cite{Brock2018Biggan,karras2019style,tewari2020stylerig,tewari2020pie}. 
% 
The quantitative results are in Table \ref{table:appearance}. Our method outperforms other baselines significantly in terms of quality of the image (FID), while maintaining diversity. 
% 



\noindent
\textbf{User Study.}
We perform a comprehensive user study to access visual fidelity and characteristics of the results between VUnet and our method for appearance sampling, as those arguably generate visually most realistic human images (see Table \ref{table:appearance}). To this end, we use $20$ random test poses and choose the results by both the methods which look most realistic, in our opinion. % 
Users are then shown a pair of generated images from the two methods for 12 poses and asked to select the most realistic one among them. Since such comparisons on individual images can be biased, we also ask the participants to decide between image sets (two to four images) for eight poses. The purpose of those is to compensate for the possible image selection biases associated with image pairs. 
% by selecting up to four best generated images. 
In the total of $36$ respondents, our method is preferred over VUnet in $\bf 91.06\%$ of the cases.




\subsection{Pose Transfer} 
\label{sec:res:posetransfer} 
In this section, we evaluate how our system preserves the appearance of the outputs across different poses and  perform the following pose transfer experiment, \textit{i.e.,} re-rendering of a subject under different poses and viewpoints. 
% 
We encode the appearance $\bm T$ of the input image $\bm I$ by using the mean of the distribution predicted by the encoder, \textit{i.e.,} $\bm z = \bm \mu$ where $\bm \mu, \bm \sigma = E(\bm T)$. 
% 
We keep $\bm z$ \textit{fixed}, and use \textit{different target poses} to generate images for pose transfer. 
% 

\begin{figure*}[t]
    % \includegraphics[width=\linewidth]{Figures/SOA.pdf} 
    \includegraphics[width=\linewidth]{Figures/garment_transfer.jpg}
    \caption{The results of our method for garment transfer. By combining the appearance encoding of two images based on the body parts, we can perform garment transfer.} 
    \label{fig:garments} 
    \vspace{-0.3cm}
\end{figure*} 

We compare our results with five state-of-the-art pose transfer methods, namely Coordinate Based Inpainting (CBI) \cite{Grigorev2019CoordinateBasedTI}, Deformable GAN (DSC) \cite{Siarohin2019AppearanceAP}, Variational U-Net (VUNet) \cite{esser2018variational} Dense Pose Transfer (DPT) \cite{Neverova2018} and Neural Human Re-Rendering (NHRR) \cite{Sarkar2020}. For both qualitative and quantitative evaluation, we use the results of 176 testing pairs that are used in the existing work \cite{Sarkar2020,Grigorev2019CoordinateBasedTI}. The qualitative results are shown in Fig.~\ref{fig:transfer}. Note that these methods, except for VUNet, are designed explicitly for the problem of pose transfer, while our method is designed as a generative model which is capable of retaining identity across different pose. We observe that our results show better realism than the other state-of-the-art methods, and perform comparably for the problem of pose transfer. This is confirmed by the comparable LPIPS distance of our model in comparison to the other SOA methods (Table \ref{table:transfer}). The appearance consistency is also verified by our result on the walking sequences of the fashion dataset \cite{Zablotskaia2019DwNetDW} (Fig.~\ref{fig:fashion}). 



\noindent
\textbf{User Study.}
Following the existing work on pose transfer, we perform another user study for evaluating our results for this task, and compare with the method of NHRR and CBI.
%
We adapt the user study format and question types from 
% the user study in 
\cite{Sarkar2020} and show the generated results of the methods from 16 source-target pairs. The user preference for \textit{identity preservation} was found to be \textbf{ours: 65.62\%}, CBI: 21.88\%, NHRR: 12.5\%. The user preference for \textit{realism} was found to be \textbf{ours: 81.25\%}, CBI: 6.25\%,  NHRR: 12.5\%. 




\begin{table}[t]
\small
\centering
\begin{tabular}{c|c|c} 
              & Variation--Part $\uparrow$   & Variation--Rest  $\downarrow$ \\ \hline
NoParts          &  0.45     &  0.44    \\
\textbf{Ours} & 0.37  &  0.11\\    \hline
\end{tabular}
\caption{Quantitative evaluation for part sampling using mean pairwise L1 distance of the masked part. $\downarrow$ ($\uparrow$) means lower (higher) is better.}
\label{table:parts}
\vspace{-0.5cm}
\end{table}

\subsection{Part-Based Sampling} 
\label{sec:res:parts} 

We next evaluate our method for part-based sampling -- the ability to produce different plausible renderings of a body part (\textit{e.g.,} head) while keeping the rest of the body same. 
% 
To this end, we vary the vector $\bm z[k] \sim \mathcal{N}(0^{N}, I^{N}) $ corresponding to the part $k$, and keep the rest of the noise vector $\bm z[j] \mid j \neq k$ fixed, and perform the decoding on a given pose. When multiple elementary DensePose parts (\textit{e.g.,} left head, right head) correspond to one logical body part for sampling (\textit{e.g.,} head), we sample noise in all the elementary part vectors. The results are shown in Fig.~\ref{fig:parts}. 




To explicitly see how much our design choices help for part sampling, we perform a baseline experiment \textbf{NoParts} where we encode the appearance in a single vector $\bm z \sim E(\bm T) \mid \bm z \in \mathbb{Z}^{N}$ instead of part-specific vectors. We then warp this vector using the conditioning DensePose to create a noise image for the generator as described in Sec.~\ref{sec:warping}. 
We compute the following two metrics for a given part $p$: 1) \textit{Variation--Part}: mean pairwise L1 distance between the samples in the masked region (by DensePose) of the part $p$ normalized by the masked area. 2) \textit{Variation--Rest}: mean pairwise L1 distance between the samples in the masked region of all body parts excluding $p$. We compute the aforementioned metrics for the following parts: ``Head'', ``Upper body'' and ``Lower body'' for 2500 generated images and provide our result in Table \ref{table:parts}. A suitable method for part sampling should generate diverse semantically meaningful renderings of a part without changing  the rest of the body. This is confirmed by high  \textit{Variation--Part} and low \textit{Variation--Rest} in our full method in comparison to the baseline \textit{NoParts}. 

Using part-specific latent vectors allows us to naturally perform 










==> Sections/method.tex <==
%!TEX root = ../article.tex
\section{Method}
\label{sec:method}

\begin{figure*}[t] 
    \includegraphics[width=\linewidth]{Figures/pipeline2.png} 
    \caption{Overview of our method. Given a source image $I_s$, we extract human appearance in the form of a UV texture map $T_s$. Subsequently, the Encoder encodes $T_s$ to part specific latent vectors $\bm z_s$. We use the target pose $P_t$ to warp and broadcast the latent vectors to the corresponding part locations in the target image to create a noise image $Z_t$. Finally, the generator converts the noise image to a realistic image. During testing, we generate random samples by controlling the latent vectors $\bf z \in \mathcal{N}(0,1)$ and the target pose $P_t$.}
    %\caption{Overview of our method. Given a source image $I_s$ and target image pair ($I_s, I_t$), we encode the source appearance from a normalized pose independent appearance space $T_s$ to part specific latent vectors $\bf z_s$. We use the target pose $P_t$ to warp and broadcast the latent vectors to the corresponding part locations in the target image and form a noise image $Z_t$. Subsequently, the generator converts the noise image to a realistic image. During testing, we generate random samples by controlling the latent vectors $\bf z \in \mathcal{N}(0,1)$ and the target pose $P_t$.} 
    \label{fig:pipeline} 
\end{figure*} 



%\begin{figure}[t] 
%    \includegraphics[width=\linewidth]{Figures/uv_texture.png} 
%    \caption{Extraction of appearance in the SMPL texture space} 
%    \label{fig:uvtexture} 
%\end{figure} 

%\paragraph{Terminology} 
%Source image, Source Pose  $I_{s}, P_{s}$
%
%Partial Texture map of the input - $T_{s}$
%
%Encoder - \textit{Enc}, E
%
%Target pose - $P_t$.
%
%Warping function - \textit{Warp, W}
%
%Sampled Noise - $\bm z$ (note that the dependence on source $s$ is dropped), tiled noise in the texture space - $T_Z$, Warped noise image - $Z_{t}$.
%
%Generator - \textit{Gen}, \textit{G}
%
%Generated image, on noise Z, and pose t - $I_{Z,t}$
%
%Pipeline can be described by the following equations:
%
%\begin{equation*}\label{eq:pareto mle2}
%  \begin{aligned}
%\mu, \sigma = E(T_s)\\
%Z \sim p(\mu, \sigma)\\
%Z_t = W(P_t, T_z)\\
%I_{Z,t} = G(Z_t)\\
% \end{aligned}
%\end{equation*}

\subsection{Method Overview}
Our goal is to learn a generative model for human images, which is conditioned on body pose and a low dimensional latent vector encapsulating the appearance \LJ{a low dimensional latent vector encapsulating the appearance -> a low dimensional latent vector where each dimension encapsulates the appearance of different body parts?}. 
We use DensePose~\cite{Guler2018DensePose} to represent the human pose because of the ease of use in terms of texture warping, and its popularity in the existing literature \cite{Siarohin2019AppearanceAP,Neverova2018,Grigorev2019CoordinateBasedTI,Sarkar2020} \LJ{should we mention why we use Densepose?}.
Our method can be described by \LJ{revised as: Our task can be formulated as?} a deterministic mapping $G':(\bm P, \bm z) \rightarrow \bm I$. Here, $\bm P \in \mathbb{R}^{H \times W \times 3}$ is a 3 channel DensePose image representing the conditioning pose, $\bm z \in \mathbb{R}^{M \times N}$ is the latent vector comprising of  $M$ human-body-parts and $N$ part-specific latent vector dimensions, and $\bm I \in \mathbb{R}^{H \times W \times 3}$ is the generated output image. 


For learning such function with a latent variable capturing the ambiguous aspect of the output, we build our method on Variational Auto-Encoder (VAE) \cite{Kingma2014VAE}. As in any latent vector model, the observed variable $\bm x$ is assumed to be dependent on an unobserved hidden latent variable $\bm z$ which encode semantically meaningful information about $\bm x$. 
%We adopt the belief that the latent variable $z$ only encode the part specific appearance. 
%The marginal distribution of the observed variable is then given by $p(I) = \int p(I, z) \,dz$. 
The goal of the generative model then is to find the distribution that maximize the marginal log-likelihood $\sum_{\bm x \in p_{\text{data}}} \log \int p_\theta(\bm x|\bm z) p(\bm z) d \bm{z}$ w.r.t. the parameters $\theta$. To make this problem tractable, a distribution $q_\phi(\bm{z|x})$ with learnable parameters, the encoder, is introduced that approximate the true but intractable posterior $p(\bm{z|x})$. With the above formulation and the Gaussian assumption on the distribution $p(\bm z)$ and $q_\phi(\bm{z|x})$, the VAE objective is to minimize $\mathcal{L}_{rec} + \mathcal{L}_{prior}$, where $\mathcal{L}_{rec}$ is the reconstruction loss, and  $\mathcal{L}_{prior}$ the KL divergence on the encoded distribution and the standard normal distribution \cite{Kingma2014VAE}. 

In this work, we use the conditional version of the VAE to learn the joint distribution $p_{\theta}(\bm{I|z})p(\bm z)$ on human images. However, we adopt the belief that the hidden latent variable $\bm z$  depends \textit{only} on the appearance of the subject in the image $\bm I$. To achieve that, our encoder takes a pose independent human appearance $\bm T$ as input, and encodes it to part specific latent vectors $\bm z$. Furthermore, the encoded appearance $\bm z$ is warped by a target pose $P_t$ different than that of $I$, which is subsequently used by a generator.

%$\mathbb{E}_{I\sim p_{\text{data}}}[\int p(I, z) \,dz]$


%The encoding of our VAE is performed on the source appearance. However, the decoding of the VAE is performed on the warped latent code on the target pose to generate a photo realistic image. Our system is composed of fours steps.
%Our system performs encoding and decoding on different spaces in order to enforce cross pose appearance consistency and part based sampling capability. 

\subsection{The Proposed Approach}
We take pairs of images ($\bm{I_s}, \bm{I_t}$) of the same person (but in different poses) as input during the training. Our method is then described by four steps. 
In the first step,  we extract SMPL \textit{UV texture map} $\bm T_{s}$ from the input image $\bm I_s$  using the DensePose correspondences. In the second step, we use an encoding function $E$ to map the human appearance $\bm T_s$ of the source image to the parameters of the distribution of the latent vector. In the third step, we sample $\bm z$  from the estimated distribution of the source appearance. Given a target pose $\bm P_t$, we warp the encoded latent vector $\bm z$ to a noise image $\bm Z_t$ (Sec.~\ref{sec:warping}). In the forth step, we decode the warped noise image $\bm Z_t$ to a realistic image $\bm I_t'$ by a high fidelity generator network. Our method is summarized in Fig. \ref{fig:pipeline}.

%We take pairs of images ($\bm{I_s}, \bm{I_t}$) of the same person (but in different poses) as input during the training. Our method is described by four steps. 
%In the first step,  we extract SMPL \textit{UV texture map} $\bm T_{s}$ from the input image $\bm I_s$  using the Densepose correspondences (Sec. \ref{sec:texmap}). This encoding acts as a pose independent appearance of the subject in the input image. In the second step, we use an encoding function $E$ to map the human appearance $\bm T_s$ of the source image to the parameters of the distribution of the latent vector (Sec. \ref{sec:encoding}). In the third step, we sample $\bm z$  from the estimated distribution of the source appearance. Given a target pose $\bm P_t$, we warp the encoded latent vector $\bm z$ to a noise image $\bm Z_t$ (Sec. \ref{sec:warping}). In the forth step, we decode the warped noise image $\bm Z_t$ to a realistic image $\bm I_t'$ by a high fidelity generator network (Sec. \ref{sec:decoding}).

\paragraph{Extracting part-specific appearance}
\label{sec:texmap}
We use UV texture map of the SMPL surface model \cite{SMPL:2015} to represent appearance of the subject in the input image. 
%The normalized texture space provided by SMPL surface model \cite{SMPL:2015} is independent of the pose making it a good candidate for representing the appearance. 
The pixels of the input image $\bm{I_s}$ are transformed into UV space through mapping predicted by DensePose RCNN~\cite{Guler2018DensePose}. The pretrained network trained on COCO-DensePose dataset predicts  $24$ body segments and their part-specific \textit{U,V} coordinates of SMPL model. For easier mapping, the 24 part-specific UV maps are combined to form a single normalized UV texture map $\bm T_s$ in the format provided in SURREAL dataset \cite{varol17_surreal}. 
% 
This normalized (partial) texture map provides us with a pose-independent appearance encoding of the subject that is located spatially according to the body parts. The 24 regions in the texture map also provides us the placeholder for parts based noise sampling (see Sec.~\ref{sec:warping}), \textit{i.e.,} in our case, the number of body parts $M = 24$.  

\paragraph{Encoding part-specific appearance}
\label{sec:encoding}
As with VAE, we assume the distribution $q(\bm{z|T_s})$ of the latent code $\bm z$ given the appearance $\bm T_s$ to be Gaussian, $q(\bm{z|T_s}) \equiv \mathcal{N}(\bm{\mu_s, \sigma_s})$. We use a convolutional neural network $E(.)$ that takes the partial texture $\bm T_s$ as input and predicts the parameters ($\bm{\mu_s, \sigma_s}$) of the Gaussian distribution, $\bm{\mu_s, \sigma_s} \in \mathbb{R}^{M \times N}$.
The encoder comprises of a convolutional layer, 5 residual blocks, an average pooling layer, and finally a fully connected layer that produces the final output.
% The encoded appearance is then used to sample the noise vector subsequently warped and used by a decoder.

\paragraph{Warping latent space}
\label{sec:warping}
In the next step, we sample a latent code from the predicted distribution of the encoded appearance, $\bm z_s \sim E(\bm T_s) \equiv \mathcal{N}(\bm{\mu_s, \sigma_s})$. 
Given the  noise vector $\bm z_s$ and a target pose $\bm P_t$, 
we intend to reconstruct a realistic image $\bm \tilde I_t$ with the appearance encoded in  $\bm z_s \in \mathbb{R}^{M \times N}$ and pose from $\bm P_t$. We also want the latent code for a specific body part to have direct influence on the same body part in the generated image. We enforce this by warping and broadcasting the part based latent code to the corresponding part location in the target image and create a noise image $\bm Z_t \in \mathbb{R}^{H \times W \times N}$. Here, for each body part $k$, $\forall_{i,j \in k} \bm Z_t[i,j] \gets \bm z[k]$ (See the warping module in Fig. \ref{fig:pipeline}). This operation can be easily implemented by differentiable sampling given the DensePose image $P_t$. The design enables us to perform part based sampling during the test time. Other straightforward ways of using the noise vector, such as sampling noise in the UV texture space, tiling of a single noise vector in the entire spatial dimension, etc. did not give us the required result. See Sec.~\ref{sec:res:appearance} and \ref{sec:res:parts}  for a detailed analysis.


\paragraph{Decoding to a Photo-Realistic image}
\label{sec:decoding}
The warped noise image in the target pose $\bm Z_t$ with the noise vectors correctly aligned with the body parts in the target pose, is used as an input to a generator network $G(.)$. The generator along with the warping module acts as the conditional decoder of our pipeline. We use the high fidelity generator from Pix2PixHD \cite{wang2018pix2pixHD} that comprises of a 3 down-sampling blocks, 6   residual blocks and a 3 up-sampling blocks for this purpose.

%Note that, we are encoding the appearance 

%The discriminator for adversarial training of RenderNet also uses the multiscale design of Pix2PixHD . In our experiments, we use a three scale discriminator network for adversarial training. 


\subsection{Training Details}
\label{sec:training}
%During the training, our system takes source-target pairs images ($\bm{I_s}, \bm{I_t}$) of the same person in different poses. The corresponding poses ($\bm{P_s}, \bm{P_t}$) is directly computed from the input images by a pretrained DensePose RCNN. The appearance in the form of UV texture map $\bm T_s$ is then extracted from the source image and passed through the encoder $E(.)$. The sampled noise $\bm z_s$ from the encoder is warped as $\bm Z_t$ using the target pose $\bm{P_t}$, and passed through the translation network $G(.)$ that acts as a decoder.
%Our system performs encoding in the normalized texture space, but it performs decoding in the target pose space. 
Our entire training pipeline can be summarized by the following equations.

\begin{equation}\label{eq:sampling}
  \begin{aligned}
\bm z_s \sim E(\bm T_s), \qquad \bm{\tilde I_{t}} = G(\bm Z_t),\\
 \end{aligned}
\end{equation}

where $\bm Z_t = W(\bm z_s, \bm P_t)$ and $W(.)$  the differentiable warping function as described in Sec.~\ref{sec:warping}.
With the re-parameterization trick \cite{Kingma2014VAE} for sampling $z_s$, the entire pipeline becomes differentiable allowing direct back-propagation to the parameters of $E(.)$ and $G(.)$. The pipeline is trained with an objective $\mathcal{L}_{total}$ derived from Conditional VAE-GAN:

\begin{equation}\label{eq:loss}
 \mathcal{L} =  \mathcal{L}_{rec} +  \mathcal{L}_{GAN} +  \mathcal{L}_{prior}
\end{equation}

The three loss terms, $\mathcal{L}_{rec}, \mathcal{L}_{GAN}$ and $\mathcal{L}_{prior}$ are described below.

\vspace{-0.3cm}
\paragraph{Reconstruction Loss}:
The reconstruction loss $\mathcal{L}_{rec}= \lambda_{VGG} L_{VGG} + \lambda_{face}L_{face}$ quantifies the dissimilarity between generated image $\bm {\tilde I_t}$ and the ground truth image $\bm I_t$. It comprises of the following terms.
\vspace{-0.2cm}
\begin{itemize}[leftmargin=*]
\itemsep-0.2em
\item \textit{Perceptual Loss}: We use perceptual loss, which is the difference between the activations on different layers of the pre-trained VGG network \cite{simonyan2014very} applied on the generated image and the ground truth image.
$L_{VGG} = \sum \frac{1}{N^j}|l^j(\bm {\tilde I_t}) - l^j(\bm I_t)|_1$.
% 
Here, $l^j$ is the activation and $N^j$ the number of elements of the j-th layer in the ImageNet pre-trained VGG network. 

\item \textit{Face Identity Loss} To better preserve facial identity, we use a pre-trained network SphereFaceNet \cite{liu2017sphereface} $S_{face}(.)$ on the cropped 
face of the generated image and the ground truth image, $L_{face} = |S_{face}(\bm I_{t}) - S_{face}(\bm {\tilde I_t})|_1.$
\end{itemize}

%The total reconstruction loss is then $$\mathcal{L}_{rec}= \lambda_{VGG} L_{VGG} + \lambda_{face}L_{face}.$$
\vspace{-0.3cm}
\paragraph{GAN Loss -- $\mathcal{L}_{GAN}$}: The GAN loss $\mathcal{L}_{GAN}= \lambda_{D} L_D + \lambda_{FM}L_{FM}$ pushes the generator to generate realistic images. We use the multiscale discriminator architecture $D$ from Pix2PixHD \cite{wang2018pix2pixHD} for implementing the GAN loss. The network $D$ is conditioned on both the generated image and warped noise image at different scales. The total GAN loss  comprises of the following terms.
\vspace{-0.2cm}
\begin{itemize}[leftmargin=*]
\itemsep-0.2em
\item \textit{Multiscale adversarial loss} We use 2 scale discriminator the adversarial loss $L_D$. 
%$D = (D_1, D_2, D_3)$ operating on different scales.
%
%$$ \mathcal{L}_{D} = \operatorname*{min}\limits_{G} \operatorname*{min}\limits_{D_1, D_2, D_3} \sum_{i = 1, 2, 3} L_{GAN}(G, D_i)$$
\item \textit{Discriminator FM loss}: We use a discriminator feature matching $L_{FM}$, which is the difference between the activations on the different layers of the discriminator applied on the generated image and the real image.
%$$\mathcal{L}_{GAN}= \lambda_{D} L_D + \lambda_{FM}L_{FM}.$$
\end{itemize}

Please refer to \cite{wang2018pix2pixHD} for more details on the adversarial loss with multiscale discriminator. 
%\KS{Describe the losses by exact formulas if you have space before the submission}.

\vspace{-0.3cm}
\paragraph{Prior loss -- $\mathcal{L}_{prior}$}:
To enable sampling at inference time, the encoding $E(\bm T_s)$ is encouraged to be close to a standard Gaussian distribution, \textit{i.e.,} the prior distribution on the $z$ vector is assumed to be $\mathcal{N}(0, I)$. Therefore, we employ the prior loss 
$\mathcal{L}_{prior} = \lambda_{KL} \mathcal{D}_{KL}(E(\bm T_s)||\mathcal{N}(0, I)),$
where $\mathcal{D}_{KL}(p||q)$ is the Kullback-Leibler divergence between the probability distributions $p(x)$ and $q(x)$. 

With re parameterization trick on sampling $\bm z_s$, we train the system end-to-end and optimize the parameters of the network $E, G$ and $D$. The final objective $\mathcal{L}_{total}$ in Eq. \ref{eq:loss} is minimized with respect to the generator $G$ and the encoder $E$, while maximized with respect to the the discriminator $D$.
We use Adam optimiser \cite{adam} for our optimization with an initial learning rate of 2$\times 10^4$, $\beta_1$ as 0.5 and no weight decay. The loss weights are set empirically to $\lambda_{VGG} = 10, \lambda_{face} = 5, \lambda_{D} = 1, \lambda_{FM} = 10, \lambda_{KL} = 0.01$. For speed, we pre-compute DensePose on the images and directly read them as input.

\begin{figure*}[t] 
    \includegraphics[width=\linewidth]{Figures/appearance_qual.jpg} 
    \caption{Result of our method for pose guided image generation, and its comparision with VUNet \cite{esser2018variational} and other baselines. The conditioning pose is shown in the left corner. Our approach produces samples of high quality than the baseline methods.} 
    \label{fig:appearance} 
\end{figure*} 


\subsection{Testing - sampling across pose and body parts}

During testing, we sample the appearance vector $\bm z$ from the prior distribution. We warp $\bm z$ with the conditioning pose $P$ and feed the resulting noise image to the trained generator $G$ to get a generated image $\bm I_{z,P}$. 

\begin{equation}\label{eq:sampling}
  \begin{aligned}
\bm z \sim \mathcal{N}(0, I), \qquad \bm{I_{z,P}} = G(\bm Z_P),\\
 \end{aligned}
\end{equation}

where $\bm Z_P = W(\bm z_, \bm P)$; $W(.)$  the warping function. The appearance $\bm z$ can be also encoded from an input image by using the encoder on its partial texture map  $\bm T$, \textit{i.e.,} $\bm z = \bm \mu$ where $\bm \mu, \bm \sigma = E(\bm T)$. Keeping $\bm z$ fixed and varying the the pose $\bm P$, we can perform pose transfer \cite{Sarkar2020,Grigorev2019CoordinateBasedTI,Siarohin2019AppearanceAP,Neverova2018} -- re-rendering a subject with different pose and viewpoint. We can also perform body parts based sampling by only varying the vector $\bm z[k]$ corresponding to the part $k$. See Sec.~\ref{sec:results} for all possible applications of our system.



